Model Selection of Anomaly Detectors in the Absence of Labeled Validation Data

Anomaly detection is the task of identifying abnormal samples in large unlabeled datasets. While the advent of foundation models has produced powerful zero-shot anomaly detection methods, their deployment in practice is often hindered by the absence of labeled validation data -- without it, their detection performance cannot be evaluated reliably. In this work, we propose SWSA (Selection With Synthetic Anomalies): a general-purpose framework to select image-based anomaly detectors without labeled validation data. Instead of collecting labeled validation data, we generate synthetic anomalies without any training or fine-tuning, using only a small support set of normal images. Our synthetic anomalies are used to create detection tasks that compose a validation framework for model selection. In an empirical study, we evaluate SWSA with three types of synthetic anomalies and on two selection tasks: model selection of image-based anomaly detectors and prompt selection for CLIP-based anomaly detection. SWSA often selects models and prompts that match selections made with a ground-truth validation set, outperforming baseline selection strategies.

==> tables/clip-prompt-results-10.tex <==
\begin{table*}[tb!]
	\centering
 \small
	\caption{Synthetic outliers can effectively select CLIP prompts in the absence of real validation data. We compare five methods for selecting CLIP prompts: (i) our method (described in \Cref{sec:prompt_selection}), (ii) a random choice of candidate prompt, (iii) always choosing the default prompt, (iv) our method with Tiny-ImageNet as the synthetic anomalies, and (iv) the single, global best candidate prompt an oracle would provide (grayed out as this cannot be obtained in practice).
    For each method, we record the tasks where the selected prompt matches the best task-specific prompt, reporting the accuracy and raw count (in parentheses) for the one-vs-one closest and one-vs-one average benchmarks.
    Across three datasets and two benchmarks, our method outperforms all other strategies, and even outperforms the global best prompt in three out of six cases.}
	\label{table:clip-prompts}
	\begin{tabular}{rr |rr rr rr rr}
	\toprule
    & & \multicolumn{2}{c}{\makecell[c]{Flowers\\(102 tasks)}} 
    & \multicolumn{2}{c}{\makecell[c]{CUB\\(200 tasks)}} 
    & \multicolumn{2}{c}{\makecell[c]{MVTec-AD\\(15 tasks)}} 
    & \multicolumn{2}{c}{\makecell[c]{VisA\\(12 tasks)}} \\
    \midrule
	\multirow{6}{*}{\makecell[c]{Closest\\Task}} 
    & Random & 10.0\% & & 10.0\% & & 10.0\% & & 10.0\% & \\
    & Default & 0.0\% & (1) & 2.5\% & (5) & 6.7\% & (1) & 0.0\% & (0) \\
    & TinyImg & 17.6\% & (18) & 17.0\% & (34) & 6.7\% & (1) &  16.7\% & (2) \\
    & CutPaste & 17.6\% & (18) & 17.0\% & (34) & 13.3\% & (2) &  \textbf{33.3\%} & (4) \\
    & Best (Oracle) & \textcolor{gray}{41.2\%} & \textcolor{gray}{(42)} & 
    \textcolor{gray}{18.5\%} & \textcolor{gray}{(37)} & \textcolor{gray}{26.7\%} & \textcolor{gray}{(4)} & 
    \textcolor{gray}{25.0\%} & \textcolor{gray}{(3)} \\
    \cmidrule(r){2-10}
        & Ours & \textbf{37.2\%} & (38) & \textbf{23.0\%} & (46) & \textbf{40.0\%} & (6) & 8.3\% & (1) \\
    \midrule
	\multirow{6}{*}{\makecell[c]{Average\\Task}} 
    & Random & 10.0\% & & 10.0\% & & 10.0\% & & 10.0\% & \\
    & Default & 0.0\% & (1) & 0.0\% & (0) & 6.7\% & (1) & 0.0\% & (0) \\
    & TinyImg & 17.6\% & (18) & 13.5\% & (27) & 6.7\% & (1) & \textbf{16.7\%} & (2) \\
    & CutPaste & 23.5\% & (24) & 12.5\% & (25) & 13.3\% & (2) & \textbf{16.7\%} & (2) \\
    & Best (Oracle) & \textcolor{gray}{44.1\%} & \textcolor{gray}{(45)} & 
    \textcolor{gray}{32.5\%} & \textcolor{gray}{(65)} & \textcolor{gray}{40.0\%} & \textcolor{gray}{(6)} & 
    \textcolor{gray}{33.3\%} & \textcolor{gray}{(4)} \\
    \cmidrule(r){2-10}
    & Ours & \textbf{40.2\%} & (41) & \textbf{32.0\%} & (64) & \textbf{46.7\%} & (7) & \textbf{16.7\%} & (2) \\
\bottomrule
\end{tabular}
\end{table*}

% Real counts (of 10): 
% Flowers 38, 41
% Flowers-TI 18, 18
% CUB 46, 64
% CUB-TI 34, 27 
% MVTec 6, 7
% MVTec-TI 6, 7

% Best prompts (of 10): 
% Flowers 42, 45 
% CUB 37, 65
% MVTec 4, 6


==> tables/clip-prompt-results-aucs.tex <==
\begin{table*}[tb!]
    \centering
    \small
    \caption{When using our synthetic outliers for CLIP prompt selection, we report both the accuracy in picking the best prompt (``pick rate'') and the resulting AUROC. \name~picks the best prompt most often and produces higher AUROCs than baseline prompt selection techniques for all datasets. \todo{Include best prompt as an oracle result, possibly merge Table 1 and 2}}
    \label{table:clip-prompts-aucs}
    \begin{tabular}{rr |cc cc cc cc}
        \toprule
        &  & \multicolumn{2}{c}{\makecell[c]{Flowers}} 
        & \multicolumn{2}{c}{\makecell[c]{CUB}} 
        & \multicolumn{2}{c}{\makecell[c]{MVTec-AD}} 
        & \multicolumn{2}{c}{\makecell[c]{VisA}} \\
        %\midrule
        & & Pick rate & AUROC & Pick rate & AUROC & Pick rate & AUROC & Pick rate & AUROC \\
        \midrule
    	\multirow{5}{*}{\makecell[c]{One-vs-Closest\\(prompt selection)}} 
        & Default Prompt & 1 / 102 & 0.697 & 5 / 200 & 0.571 & 1 / 15 & 0.540 & 1 / 12 & 0.491 \\
        & Prompt Ensemble & -- & 0.708 & -- & 0.577 & -- & 0.555 & -- & 0.494 \\
        %& Worst Prompt (Oracle) & \textcolor{gray}{0.658} & \textcolor{gray}{0.394} & \textcolor{gray}{0.386} & \textcolor{gray}{0.394} \\
        % & Best Prompt (Oracle) & & \textcolor{gray}{0.759} & & \textcolor{gray}{0.578} & & \textcolor{gray}{0.684} & & \textcolor{gray}{0.578} \\
          & SWSA (TinyImg) & 18 / 102 & 0.718 & 34 / 200 & 0.582 & 1 / 15 & 0.559 & 4 / 12 & 0.514 \\
          & SWSA (Diffusion) & 38 / 102 & \textbf{0.729} & 46 / 200 & \textbf{0.590} & 3 / 15 & 0.529 & 1 / 12 & 0.475 \\
          & SWSA (CutPaste) & 18 / 102 & 0.718 & 34 / 200 & 0.585 & 4 / 15 & \textbf{0.609} & 1 / 12 & \textbf{0.507} \\
         %    \midrule
        	% \multirow{5}{*}{\makecell[c]{One-vs-One\\Average}} 
         %    & Default Prompt & 1 / 102 & 0.955 & 0 / 200 & 0.971 & 1 / 15 & 0.691 & 1 / 12 & 0.635 \\
         %    & Prompt Ensemble & 3 / 102 & 0.958 & 0 / 200 & 0.972 & 0 / 15 & 0.711 & 0 / 12 & 0.656 \\
         %    %& Worst Prompt (Oracle) & \textcolor{gray}{0.948} & \textcolor{gray}{0.964} & \textcolor{gray}{0.607} & \textcolor{gray}{0.571} \\
         % & Best Prompt (Oracle) & & \textcolor{gray}{0.968} & & \textcolor{gray}{0.976} & &\textcolor{gray}{0.781} & & \textcolor{gray}{0.706} \\
         %      & SWSA (TinyImg) & 18 / 102 & \textbf{0.964} & 27 / 200 & 0.972 & 1 / 15 & 0.703 & 6 / 12 & 0.659 \\
         %      & SWSA (Diffusion) & 41 / 102 & \textbf{0.964} & 64 / 200 & \textbf{0.973} & 2 / 15 & 0.692 & 3 / 12 & 0.632 \\
         %      & SWSA (CutPaste) & 24 / 102 & 0.959 & 25 / 200 & 0.972 & 5 / 15 & \textbf{0.747} & 3 / 12 & \textbf{0.666} \\
        \midrule
        \multirow{5}{*}{\makecell[c]{One-vs-Rest\\(prompt selection)}} 
        & Default Prompt & 1 / 102 & 0.959 & 0 / 200 & 0.971 & 1 / 15 & 0.641 & 2 / 12 & 0.620 \\
        & Prompt Ensemble & -- & 0.962 & -- & 0.972 & -- & 0.654 & -- & 0.641 \\
        %& Worst Prompt (Oracle) & \textcolor{gray}{0.948} & \textcolor{gray}{0.964} & \textcolor{gray}{0.607} & \textcolor{gray}{0.571} \\
        % & Best Prompt (Oracle) & & \textcolor{gray}{0.968} & & \textcolor{gray}{0.976} & & \textcolor{gray}{0.781} & & \textcolor{gray}{0.706} \\
          & SWSA (TinyImg) & 13 / 102 & \textbf{0.967} & 27 / 200 & 0.972 & 1 / 15 & 0.650 & 4 / 12 & 0.640 \\
          & SWSA (Diffusion) & 38 / 102 & \textbf{0.967} & 64 / 200 & \textbf{0.973} & 2 / 15 & 0.642 & 1 / 12 & 0.614 \\
          & SWSA (CutPaste) & 22 / 102 & 0.963 & 27 / 200 & 0.972 & 5 / 15 & \textbf{0.684} & 4 / 12 & \textbf{0.644} \\
    	\bottomrule
\end{tabular}
\end{table*}


==> tables/model-selection-aucs.tex <==
\begin{table*}[tb!]
	\centering
 \small
	\caption{When using synthetic anomalies for model selection, we report both the accuracy in picking the best model (``pick rate'') and the resulting AUROC. \name~picks the best model more often and produces higher AUROCs than simply selecting the largest model for all tasks. Diffusion-based synthetic anomalies are particularly effective for model selection on the Flowers and CUB datasets.
 }
	\label{table:model-aucs}
	\begin{tabular}{rr |cc cc cc cc}

	\toprule
    &  
    & \multicolumn{2}{c}{\makecell[c]{Flowers}} 
    & \multicolumn{2}{c}{\makecell[c]{CUB}} 
    & \multicolumn{2}{c}{\makecell[c]{MVTec-AD}} 
    & \multicolumn{2}{c}{\makecell[c]{VisA}} \\
    %\midrule
    & & Pick rate & AUROC & Pick rate & AUROC & Pick rate & AUROC & Pick rate & AUROC \\
    \midrule
	\multirow{4}{*}{\makecell[c]{One-vs-Closest\\(model selection)}} 
    & Largest model & 43 / 102 & 0.956 & 11 / 200 & 0.653 & 4 / 15 & 0.716 & 1 / 12 & 0.636 \\
    & SWSA (TinyImg) & 50 / 102 & 0.966 & 30 / 200 & 0.674 & 4 / 15 & 0.716 & 1 / 12 & 0.636 \\
    & SWSA (Diffusion) & 59 / 102 & \textbf{0.967} & 66 / 200 & 0.737 & 4 / 15 & \textbf{0.790} & 0 / 12 & 0.643 \\
    & SWSA (CutPaste) & 37 / 102 & 0.945 & 60 / 200 & \textbf{0.743} & 2 / 15 & 0.678 & 1 / 12 & \textbf{0.674} \\
 %    \midrule
	% \multirow{4}{*}{\makecell[c]{One-vs-One\\Average}} 
 %    & Largest model & 45 / 102 & \textbf{0.977} & 32 / 200 & 0.983 & 4 / 15 & \textbf{0.825} & 1 / 12 & 0.787 \\
 %    & SWSA (TinyImg) & 53 / 102 & 0.973 & 57 / 200 & 0.982 & 4 / 15 & 0.825 & 1 / 12 & 0.787 \\
 %    & SWSA (Diffusion) & 63 / 102 & \textbf{0.977} & 108 / 200 & \textbf{0.988} & 2 / 15 & 0.706 & 0 / 12 & 0.787 \\
 %    & SWSA (CutPaste) & 36 / 102 & 0.927 & 60 / 200 & 0.966 & 2 / 15 & 0.804 & 1 / 12 & \textbf{0.794} \\
    \midrule
	\multirow{4}{*}{\makecell[c]{One-vs-Rest\\(model selection)}} 
    & Largest model & 49 / 102 & \textbf{0.994} & 32 / 200 & 0.982 & 4 / 15 & \textbf{0.733} & 1 / 12 & 0.765 \\
    & SWSA (TinyImg) & 57 / 102 & 0.993 & 59 / 200 & 0.982 & 4 / 15 & 0.733 & 1 / 12 & 0.765 \\
    & SWSA (Diffusion) & 62 / 102 & \textbf{0.994} & 109 / 200 & \textbf{0.988} & 2 / 15 & 0.678 & 0 / 12 & 0.764 \\
    & SWSA (CutPaste) & 37 / 102 & 0.974 & 62 / 200 & 0.966 & 2 / 15 & 0.717 & 1 / 12 & \textbf{0.772} \\
    
 \bottomrule
\end{tabular}
\end{table*}

 %    & Largest model & 43 / 102 & 11 / 200 &  4 / 15 & 1 / 12 \\
 %    & Selected with Tiny-Imagenet & 50 / 102 & 30 / 200 &  4 / 15 & 1 / 12 \\
 %    & Selected with Diffusion-generated Anomalies & 59 / 102 & 66 / 200 & 4 / 15 & 0 / 12 \\
 %    & Selected with CutPaste-generated Anomalies & 37 / 102 & 60 / 200 & 2 / 15 & 1 / 12 \\
 %    \midrule
	% \multirow{4}{*}{\makecell[c]{One-vs-One\\Average}} 
 %    & Largest model & 45 / 102 & 32 / 200 &  4 / 15 & 1 / 12 \\
 %    & Selected with Tiny-Imagenet & 53 / 102 & 57 / 200 & 4 / 15 & 1 / 12 \\
 %    & Selected with Diffusion-generated Anomalies & 63 / 102 & 108 / 200 & 2 / 15 & 0 / 12 \\
 %    & Selected with CutPaste-generated Anomalies & 36 / 102 & 60 / 200 & 2 / 15 & 1 / 12 \\
 %    \midrule
	% \multirow{4}{*}{\makecell[c]{One-vs-Rest}} 
 %    & Largest model & 49 / 102 & 32 / 200 & 4 / 15 & 1 / 12 \\
 %    & Selected with Tiny-Imagenet & 57 / 102 & 59 / 200 & 4 / 15 & 1 / 12 \\
 %    & Selected with Diffusion-generated Anomalies & 62 / 102 & 109 / 200 & 2 / 15 & 0 / 12 \\
 %    & Selected with CutPaste-generated Anomalies & 37 / 102 & 62 / 200 & 2 / 15 & 1 / 12 \\

==> tables/model-selection-rank10.tex <==
\begin{table*}[tb!]
	\centering
     \small
	\caption{Using our synthetic outliers to select models results in the best average AUROC, even in the absence of real validation data. \todo{Merge into Table 2}}
	\label{table:model-ranks}
	\begin{tabular}{rr |cccc}
	\toprule
    & & \makecell[c]{Flowers\\(102 tasks)} 
    & \makecell[c]{CUB\\(200 tasks)} 
    & \makecell[c]{MVTec-AD\\(15 tasks)} 
    & \makecell[c]{VisA\\(12 tasks)} \\
    \midrule
	\multirow{4}{*}{\makecell[c]{One-vs-One\\Closest}} 
    & Largest model & 43 / 102 & 11 / 200 &  4 / 15 & 1 / 12 \\
    & Selected with Tiny-Imagenet & 50 / 102 & 30 / 200 &  4 / 15 & 1 / 12 \\
    & Selected with Diffusion-generated Anomalies & 59 / 102 & 66 / 200 & 4 / 15 & 0 / 12 \\
    & Selected with CutPaste-generated Anomalies & 37 / 102 & 60 / 200 & 2 / 15 & 1 / 12 \\
    \midrule
	\multirow{4}{*}{\makecell[c]{One-vs-One\\Average}} 
    & Largest model & 45 / 102 & 32 / 200 &  4 / 15 & 1 / 12 \\
    & Selected with Tiny-Imagenet & 53 / 102 & 57 / 200 & 4 / 15 & 1 / 12 \\
    & Selected with Diffusion-generated Anomalies & 63 / 102 & 108 / 200 & 2 / 15 & 0 / 12 \\
    & Selected with CutPaste-generated Anomalies & 36 / 102 & 60 / 200 & 2 / 15 & 1 / 12 \\
    \midrule
	\multirow{4}{*}{\makecell[c]{One-vs-Rest}} 
    & Largest model & 49 / 102 & 32 / 200 & 4 / 15 & 1 / 12 \\
    & Selected with Tiny-Imagenet & 57 / 102 & 59 / 200 & 4 / 15 & 1 / 12 \\
    & Selected with Diffusion-generated Anomalies & 62 / 102 & 109 / 200 & 2 / 15 & 0 / 12 \\
    & Selected with CutPaste-generated Anomalies & 37 / 102 & 62 / 200 & 2 / 15 & 1 / 12 \\
 \bottomrule
\end{tabular}
\end{table*}


==> tables/tables-corr.tex <==

% Note: This table deprecated in favor of tables-kendallrank
\begin{table}[tb!]
	\centering
	\caption{For the model ranking results shown in \Cref{fig:model-selection-scatter}, we show the Kendall's Tau 
    rank correlation between the rankings with the synthetic and real validation datasets.}
	\label{table:corr}
	\begin{tabular}{rr|cc}
	\toprule
    && w/ Diffusion & w/ Cutpaste \\
    \midrule
    \multirow{4}{*}{\makecell[c]{One-vs\\Closest}} 
    & CUB & 0.691 & 0.790 \\ 
    & Flowers & \textbf{0.978} & 0.872 \\ 
    & MVTec-AD & 0.157 & 0.545 \\ 
    & VisA & 0.910 & 0.686 \\ 
    \midrule
    \multirow{4}{*}{\makecell[c]{One-vs\\Rest}} 
    & CUB & \textbf{0.985} & 0.709 \\ 
    & Flowers & \textbf{0.970} & 0.890 \\ 
    & MVTec-AD & 0.034 & 0.487 \\ 
    & VisA & 0.854 & 0.656 \\ 
    \bottomrule
    \end{tabular}
\end{table}
